RECALL: Recovery Experience Collection for Active Lifelong Learning in Vision-Language-Action Models

Vision-Language-Action (VLA) models are commonly fine-tuned through passive imitation learning, where additional demonstrations are collected for tasks where the policy performs poorly. This approach incurs several downsides: it requires the robot to fail before data collection is triggered, provides little guidance about which states require supervision, and wastes demonstrator effort on redundant parts of the task where the policy already performs well. In this paper, we propose an active, continual learning paradigm for VLAs. We demonstrate that active, uncertainty-guided data collection leads to more efficient fine-tuning than when using passively-collected demonstrations. However, we also find that fine-tuning only on actively-collected recovery data leads to catastrophic forgetting. We evaluate techniques for continual learning, including replay-based data mixing and elastic weight consolidation, and identify tradeoffs between plasticity to uncertainty-guided recovery data and retention of previously learned behaviors. Overall, our work contributes an empirical study of active continual learning for autoregressive VLAs, establishing that uncertainty-guided recovery demonstrations can improve adaptation efficiency while also revealing open challenges when targeted new data is incorporated into large robot policies.

==> conclusion.tex <==
% We studied active continual learning for autoregressive vision-language-action models. Instead of passively collecting additional demonstrations from task initial states after poor performance is observed, we use INSIGHT help predictions to identify uncertain, policy-induced states and collect recovery demonstrations from those states. Our results show that uncertainty-guided recovery demonstrations are more informative than matched passive start-state recollection: when mixed with prior demonstration data, they improve LIBERO-10 performance more efficiently while preserving retained-task behavior.

% At the same time, our experiments show that targeted data collection creates a continual-learning challenge. Recovery demonstrations are useful precisely because they focus on difficult states, but this narrow distribution makes new-only fine-tuning unstable and leads to catastrophic forgetting. We find that replay-based data mixing provides the most reliable solution among the methods tested, while low learning rates and EWC reduce forgetting but limit adaptation. We further show that replay scope matters: replaying LIBERO-10 demonstrations recovers most of the benefit of full prior-data replay, while replaying only collected-task data can degrade non-collected tasks.

% Overall, these findings suggest that VLA adaptation should be framed as active continual learning. A robot policy should not only detect when it needs help, but also use those moments to collect informative experience and incorporate that experience without erasing prior skills. This points toward future VLA systems that improve through repeated cycles of deployment, uncertainty-guided intervention, recovery-data collection, and stable continual adaptation.
We studied active continual learning for autoregressive vision-language-action models by using INSIGHT help predictions to identify high-uncertainty, policy-induced states and collect recovery demonstrations from those states. Our experiments show that these uncertainty-guided demonstrations are more informative than matched passive start-state collection when mixed with prior data, improving LIBERO-10 performance while preserving retained-task behavior. However, targeted recovery data also creates a continual-learning challenge: new-only fine-tuning causes catastrophic forgetting, while low learning rates and EWC improve stability but limit adaptation. Among the strategies we evaluated, replay-based data mixing provides the most reliable stability-plasticity tradeoff, with replay scope strongly affecting whether non-collected tasks are preserved. Overall, our results suggest that VLA adaptation should be framed as active continual learning, where robots not only detect when they need help, but also use those moments to collect informative experience and integrate it without erasing prior skills.

==> discussion.tex <==
Our experiments suggest that active learning for VLAs is most naturally understood as an active continual learning problem. The central challenge is not only identifying informative states for additional supervision, but also integrating the resulting targeted data without degrading previously learned behaviors. We summarize the main takeaways below.

\paragraph{Uncertainty-guided recovery states are more informative than passive task starts.}
When controlling for task distribution and number of new demonstrations, recovery demonstrations collected from INSIGHT-flagged states improve performance more than passive demonstrations collected from task initial states. This suggests that the benefit of active data collection is not simply due to adding more data, but due to collecting data at states where the policy is predicted to require assistance. In long-horizon manipulation tasks, many states in a full demonstration may already be well represented by the original training data; uncertainty-guided recovery collection instead concentrates supervision on states that are more likely to expose the model's weaknesses.

\paragraph{The first reliable uncertainty event is an efficient intervention point.}
We find that first-flag collection performs comparably to, and in some cases better than, all-flag collection despite requiring fewer recovery demonstrations. This suggests that the earliest state at which the policy appears uncertain may be especially valuable: it may correspond to the point where the rollout begins to diverge from successful behavior. Collecting a corrective demonstration from this point can provide supervision for both the uncertain state and the remainder of the task. Dense offline collection from all flagged states may add more data, but does not necessarily add proportionally more useful data.

\paragraph{Help-predictor transfer matters.}
We use Strong INSIGHT as the main uncertainty signal because it provides the cleaner transfer setting: the help predictor is trained from broader real-world rollout data and transferred to LIBERO, rather than being trained directly on LIBERO simulation data. Weak INSIGHT provides a useful comparison, but the prior INSIGHT evaluation shows that the sim-only weakly supervised model is effectively in-domain for the simulated LIBERO setting, while the strongly supervised jumbo model approaches its performance despite being trained on real-world data. This distinction matters because active data collection should ideally work without requiring task-specific help labels in the target domain.

\paragraph{Recovery data alone is not enough.}
Although uncertainty-guided recovery demonstrations are informative, fine-tuning only on this new data causes catastrophic forgetting. This is expected in retrospect: the new recovery dataset is intentionally narrow, since it is collected from difficult and policy-induced states rather than from the full task distribution. As a result, it does not provide enough coverage to preserve the behaviors that the original policy already performs well. Active learning for VLAs therefore cannot be reduced to selecting high-value states; the adaptation procedure must also preserve prior competence.

\paragraph{Replay currently provides the best stability-plasticity tradeoff.}
Among the continual-learning strategies we evaluate, replay-based data mixing most reliably balances adaptation and retention. Mixing recovery demonstrations with prior data preserves retained-task performance while allowing the model to benefit from targeted recovery supervision. In contrast, low learning rates and EWC can reduce forgetting, but often do so by limiting plasticity. Strong regularization preserves prior behavior but prevents the policy from adapting sufficiently to the new recovery data. This suggests that, at least for current autoregressive VLA fine-tuning, data-level replay is more effective than parameter regularization alone.

\paragraph{Replay coverage matters.}
Replay does not necessarily need to include the entire original dataset, but it must cover the behaviors that should be retained. Restricting replay to LIBERO-10 preserves most of the benefit of full replay, while replaying only the tasks for which recovery data was collected causes degradation on non-collected tasks. This indicates that the replay distribution is itself a design choice: it should include both the states targeted for improvement and the behaviors that should remain stable.

==> evaluation.tex <==
\todo{give an overview of the different experimental conditions you evaluate}

\subsection{Passive Start-State Recollection Baseline}
\label{sec:passive_baseline}

To isolate the value of uncertainty-guided state selection, we compare against passive recollection baselines. These baselines collect additional demonstrations from the original task initial-state distribution rather than from uncertainty-flagged states. We match the passive baseline to the uncertainty-guided data in terms of task distribution and number of collected demonstrations. This comparison controls for the possibility that improvements come simply from adding more task-relevant demonstrations, rather than from collecting demonstrations at states where the policy is uncertain.

We denote the passive recollection dataset by $\mathcal{D}_{\mathrm{passive}}$. Unlike $\mathcal{D}_{\mathrm{rec}}$, whose trajectories begin from states induced by the learned policy, trajectories in $\mathcal{D}_{\mathrm{passive}}$ begin from standard task initial states. Comparing models trained with $\mathcal{D}_{\mathrm{rec}}$ and $\mathcal{D}_{\mathrm{passive}}$ allows us to evaluate whether uncertainty-guided recovery data is more informative than matched passive data collection.

\subsection{Evaluation Protocol}
\label{sec:evaluation_protocol}

We evaluate all adapted policies on LIBERO-10 using the same rollout protocol as the baseline policy. Each policy is evaluated across the full task suite, and we report both overall success rate and per-task success rate. Overall success measures whether adaptation improves benchmark-level performance, while per-task success allows us to distinguish improvements on tasks targeted by recovery collection from degradation on non-targeted tasks. Since recovery data is collected for only a subset of LIBERO-10 tasks, we also analyze collected-task and non-collected-task performance separately.

To compare uncertainty-guided collection against passive recollection, we evaluate models trained with matched task and data distributions. To analyze continual-learning behavior, we compare performance across new-only fine-tuning, replay-based data mixtures, and EWC-regularized training. 
%We use statistical tests for differences in success rates and report whether improvements over the baseline and matched passive recollection are statistically significant.


==> problem_definition.tex <==
Overall, active learning in VLAs remains an unsolved and under-explored challenge. In this work, we propose an active, continual learning paradigm for fine-tuning VLAs. We focus on autoregressive VLAs, particularly $\pi_0$-FAST~\citep{fast}, which tokenizes continuous robot action sequences and predicts them with a next-token objective.

\textbf{Toward enabling active learning} in VLAs, we leverage INSIGHT for uncertainty quantification~\citep{karli2025insightinferencetimesequenceintrospection} and operationalize it by interpreting its ``help predictions'' as a proxy for high-uncertainty states from which to collect new demonstrations. 
%prompt active data collection in states where the policy is uncertain about how to behave. By targeting states where the model internally signals that it needs help, we aim to 
%collect demonstrations starting from states in which the policy is uncertain about how to act. %We use INSIGHT by interpreting its ``help predictions'' as a proxy for high-uncertainty states.
We study whether uncertainty-guided data collection enables effective active learning, leading to our first research question \textbf{RQ-1:} Compared to passive data collection, do demonstrations originating from high-uncertainty states result in better policy performance?

We next consider the effect of online vs offline active learning in VLA performance. In online learning, the robot requests a demonstration in real-time, which thus originates at the \emph{first} uncertain state within a policy rollout. In contrast, an offline learning setting involves the robot performing a full rollout of the task, recording \emph{every} uncertain state to revisit and prompt demonstrations at a later time. We pose \textbf{RQ-2:} Is online-style data collection sufficient, or do we need dense offline collection from all uncertain states?

%For these first two questions, we perform active learning with dataset aggregation; i.e., the model is trained over a combination of the robot's pre-existing dataset and the newly-collected, uncertainty-guided data. 
\textbf{Toward \emph{continual} active learning} for VLAs, we evaluate \textbf{RQ-3:} Can autoregressive VLAs be fine-tuned \emph{only} on newly collected recovery data? This is in contrast to the dataset aggregation assumed for RQ-1\&2, which combine the robot's pre-existing dataset and the newly-collected, uncertainty-guided data.
Finally, we apply and evaluate standard techniques for continual learning to address \textbf{RQ-4:} Do data replay and/or regularization methods mitigate catastrophic forgetting while still enabling adaptation to new training data?

%This formulation casts robot control as sequence modeling and enables introspection over the action-generation process itself. 

%We study active continual adaptation for an autoregressive vision-language-action policy $\pi_\theta$. 
%In autoregressive VLAs such as $\pi_0$-FAST, continuous action chunks are tokenized and trained with a next-token prediction objective. 

%Given an initial demonstration dataset $\mathcal{D}_{\mathrm{old}}$ and a baseline policy trained on this dataset, our goal is to fine-tune the policy by collecting an additional dataset $\mathcal{D}_{\mathrm{new}}$, with the objective of improving its task success while preserving the capabilities of the original policy.

%The standard passive adaptation strategy collects new demonstrations from task initial states. In contrast, we consider an active setting where new demonstrations are collected from states where the policy is predicted to be uncertain or likely to require assistance. 

%This produces a continual-learning problem: the newly collected data may be more informative than passive demonstrations, but it may also differ from the original training distribution and cause forgetting if used for fine-tuning in isolation.

%We address the following Research Questions (RQs):
%\begin{itemize}[leftmargin=*]
%    \item \textbf{RQ-1:} Are uncertainty-flagged states better data collection targets than passive task start states?
%    \item \textbf{RQ-2:} Is online-style intervention sufficient, or do we need dense offline collection from all uncertain states?
%    \item \textbf{RQ-3:} Can autoregressive VLAs be fine-tuned only on newly collected recovery data?
%    \item \textbf{RQ-4:} What prevents forgetting while preserving adaptation?
%    \item \textbf{RQ-5:} How much old data is necessary?
%\end{itemize}



==> results.tex <==
We evaluate whether uncertainty-guided recovery demonstrations improve autoregressive VLA fine-tuning more efficiently than passive recollection, and whether targeted recovery data can be incorporated without catastrophic forgetting. All policies are evaluated on LIBERO-10 with 50 rollouts per task, for a total of 500 rollouts per checkpoint. We report three metrics: \textit{overall} success across all tasks, \textit{collected-task} success on the tasks used for recovery-data collection, and \textit{retained-task} success on the remaining tasks. The collected tasks are tasks 2, 3, 5, 8, and 9, while tasks 0, 1, 4, 6, and 7 are treated as retained tasks. The original baseline policy achieves 58.4\% overall success, with 27.6\% success on collected tasks and 89.2\% success on retained tasks. Appendix~\ref{app:additional_results} provides best-checkpoint summaries, pairwise statistical tests, and raw per-checkpoint task success counts.

We use INSIGHT~\citep{karli2025insightinferencetimesequenceintrospection} to identify states where the VLA is likely to require assistance. INSIGHT predicts help triggers from token-level uncertainty features extracted during autoregressive action decoding, including entropy, log-probability, and Dirichlet-based aleatoric and epistemic uncertainty estimates. Prior work evaluates INSIGHT under two supervision regimes: strong supervision, where each step receives a binary help label, and weak supervision, where only episode-level success or failure labels are available. We therefore refer to the corresponding help predictors as \textit{Strong INSIGHT} and \textit{Weak INSIGHT}. These terms describe the supervision used to train the help predictor, not the difficulty of the downstream LIBERO tasks.

Our main experiments use Strong INSIGHT. This is the cleaner transfer setting for active VLA learning: in the prior Sim-OOD evaluation, the sim-only weakly supervised model is trained directly on LIBERO simulation data and is therefore in-domain for the LIBERO setting, whereas the strongly supervised jumbo model is trained on broader real-world rollout data and transfers to the simulated LIBERO setting. Thus, Strong INSIGHT allows us to test whether help predictions learned outside the downstream LIBERO data distribution can still guide useful recovery-data collection. We include Weak INSIGHT as an additional comparison because it provides a useful in-domain or LIBERO-aligned reference point.

\subsection{Uncertainty-Guided Recovery Data Outperforms Passive Recollection}
\label{sec:results_active_vs_passive}

We first ask whether uncertainty-flagged states are better data collection targets than passive task initial states. To isolate the value of state selection, we compare uncertainty-guided recovery demonstrations against passive start-state recollection baselines matched for task distribution and number of collected demonstrations. Both datasets are mixed with prior demonstration data and used to fine-tune the same baseline VLA.

Figure~\ref{fig:rq1_active_vs_passive_strong} shows the primary comparison using Strong INSIGHT. This setting evaluates whether a help predictor trained outside the LIBERO simulation distribution can identify useful recovery states for LIBERO-10 fine-tuning. The uncertainty-guided first-flag recovery model reaches 69.8\% overall success, compared to 60.2\% for the matched passive start-state recollection baseline and 58.4\% for the original VLA. This improvement over matched passive recollection is statistically significant ($p=0.0015$). The improvement is concentrated on the collected tasks, where uncertainty-guided recovery data improves success from 27.6\% to 48.8\%, compared to 33.2\% for passive recollection. Retained-task performance remains close to the original baseline, indicating that the improvement is not achieved by sacrificing tasks that were already strong.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq1_active_vs_passive_strong.png}
    \caption{
    \textbf{Strong INSIGHT recovery data outperforms matched passive recollection.}
    Strong INSIGHT provides the main transfer setting: the help predictor is trained outside the downstream LIBERO simulation distribution, yet its flagged states produce more informative recovery demonstrations than passive task-start recollection.
    }
    \label{fig:rq1_active_vs_passive_strong}
\end{figure}

Figure~\ref{fig:rq1_active_vs_passive_weak} repeats the active-versus-passive comparison using Weak INSIGHT with old normalization statistics. In contrast to the main Strong INSIGHT setting, Weak INSIGHT is closer to an in-domain or LIBERO-aligned help signal because the corresponding sim-only variant is trained directly on LIBERO simulation data in the prior Sim-OOD evaluation. This comparison therefore tests whether the active-data-collection benefit persists when the uncertainty signal is more directly aligned with the downstream benchmark. The weak setting shows the same qualitative trend: uncertainty-guided data provides useful collected-task improvement when mixed with prior demonstrations.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq1_active_vs_passive_weak.png}
    \caption{
    \textbf{Weak INSIGHT active-versus-passive comparison with old normalization statistics.}
    Weak INSIGHT provides a complementary comparison using an episode-level help-prediction signal that is more closely aligned with the downstream LIBERO setting. The comparison tests whether uncertainty-guided collection remains useful under a different supervision regime.
    }
    \label{fig:rq1_active_vs_passive_weak}
\end{figure}

Because normalization statistics can affect VLA fine-tuning, Figure~\ref{fig:rq1_active_vs_passive_weak_new_norm} also reports the weak active-versus-passive comparison with new normalization statistics. This comparison provides a norm-matched weak setting and helps separate the effect of the help predictor from the effect of normalization. Across both weak comparisons, the results support the same qualitative conclusion as the strong setting: uncertainty-guided data collection can produce more useful demonstrations than passive start-state recollection, although we treat the weak results as complementary because the weak predictor is more LIBERO-aligned.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq1_active_vs_passive_weak_new_norm.png}
    \caption{
    \textbf{Weak INSIGHT active-versus-passive comparison with new normalization statistics.}
    This norm-matched comparison complements Figure~\ref{fig:rq1_active_vs_passive_weak} and tests whether the weak INSIGHT trend persists when both active and passive datasets are evaluated under new normalization statistics.
    }
    \label{fig:rq1_active_vs_passive_weak_new_norm}
\end{figure}

Together, Figures~\ref{fig:rq1_active_vs_passive_strong}, \ref{fig:rq1_active_vs_passive_weak}, and~\ref{fig:rq1_active_vs_passive_weak_new_norm} show that uncertainty-guided recovery collection is not merely adding more data from the same task distribution. Instead, collecting from states where the policy is predicted to require assistance produces demonstrations that more directly target the model's weaknesses.

\subsection{First-Flag Collection Is More Efficient Than All-Flag Collection}
\label{sec:results_first_vs_all}

We next compare two uncertainty-guided collection regimes. The first, online-style first-flag collection, gathers a recovery demonstration only from the first state flagged in each rollout. The second, offline-style all-flag collection, gathers demonstrations from all flagged states. The all-flag setting therefore uses denser recovery data, while the first-flag setting tests whether a single early intervention can provide sufficient corrective supervision.

We focus this comparison on Strong INSIGHT because it provides the main transfer setting. Since the strongly supervised jumbo model transfers to LIBERO from broader real-world rollout data, first-versus-all collection with Strong INSIGHT tests whether transferred help predictions are sufficient to guide efficient data collection.

Figure~\ref{fig:rq2_first_vs_all_curves} shows training curves for first-flag and all-flag recovery data mixed with prior demonstrations. First-flag collection reaches 69.8\% overall success at its best checkpoint, while all-flag collection reaches 68.4\% overall success at its best checkpoint. The two methods achieve nearly identical collected-task performance, with first-flag collection reaching 48.8\% and all-flag collection reaching 48.4\%. However, all-flag collection does not provide a clear overall advantage despite using more recovery demonstrations.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq2_first_vs_all_curves.png}
    \caption{
    \textbf{First-flag versus all-flag uncertainty-guided collection over training.}
    Using Strong INSIGHT, first-flag collection reaches comparable overall success to all-flag collection despite using fewer recovery demonstrations. Dense offline collection from all flagged states does not provide a clear overall advantage.
    }
    \label{fig:rq2_first_vs_all_curves}
\end{figure}

Figure~\ref{fig:rq2_first_vs_all_best_bars} summarizes the best checkpoint for each method. Although first-flag collection achieves the highest overall success, the difference from all-flag collection is not statistically significant ($p=0.632$). We therefore interpret this result as evidence for data efficiency rather than superiority: first-flag collection reaches comparable performance while requiring fewer recovery demonstrations. Since the first-flag setting requires fewer demonstrations, this suggests that the earliest reliable uncertainty event in a rollout may be a particularly valuable intervention point. Once the policy reaches a state where it requires assistance, a corrective demonstration from that state may provide enough information to recover the remainder of the task.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq2_first_vs_all_best_bars.png}
    \caption{
    \textbf{Best-checkpoint comparison of first-flag and all-flag recovery collection.}
    First-flag collection achieves comparable overall performance to all-flag collection while using fewer recovery demonstrations. All-flag collection improves collected-task performance but does not clearly improve overall success.
    }
    \label{fig:rq2_first_vs_all_best_bars}
\end{figure}

These results motivate using first-flag recovery collection as the primary uncertainty-guided data collection strategy in later experiments. The result also suggests that active data collection should not necessarily aim to collect every uncertain state. Instead, strategically collecting from the earliest uncertainty event may be more efficient.

\subsection{New-Only Fine-Tuning Causes Catastrophic Forgetting}
\label{sec:results_new_only_forgetting}

We then ask whether recovery demonstrations can be used alone for fine-tuning. This is an important continual-learning question. If uncertainty-guided data is highly informative, then one might hope that the model could simply fine-tune on the newly collected recovery demonstrations. However, because recovery demonstrations are collected from difficult, policy-induced states, they may differ substantially from the original training distribution.

Figure~\ref{fig:rq3_new_only_forgetting} compares new-only fine-tuning against replay-based all-mix training across Strong INSIGHT first-flag, Strong INSIGHT all-flag, and Weak INSIGHT first-flag recovery datasets. New-only fine-tuning consistently causes severe forgetting. Retained-task performance collapses as training progresses, and overall success falls far below the original baseline. In contrast, mixing the same recovery data with prior demonstrations preserves retained-task performance and enables improvement on collected tasks.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq3_new_only_forgetting.png}
    \caption{
    \textbf{New-only fine-tuning causes catastrophic forgetting across recovery-data variants.}
    We compare new-only training against replay-based all-mix training for Strong INSIGHT first-flag, Strong INSIGHT all-flag, and Weak INSIGHT first-flag recovery data. New-only fine-tuning rapidly degrades overall and retained-task performance, while replay stabilizes adaptation.
    }
    \label{fig:rq3_new_only_forgetting}
\end{figure}

Figure~\ref{fig:rq3_new_only_forgetting_strong_only} provides a cleaner view of the same effect for Strong INSIGHT. Both first-flag and all-flag new-only training degrade rapidly, while their replay-based counterparts remain stable. The best Strong INSIGHT first-flag new-only checkpoint reaches only 28.4\% overall success, with retained-task performance dropping to 56.4\% and collected-task performance nearly collapsing to 0.4\%. This shows that the forgetting effect is not specific to a particular collection density. Rather, the issue is that recovery data alone is too narrow to preserve the broad task competence of the original model.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq3_new_only_forgetting_strong_only.png}
    \caption{
    \textbf{Strong INSIGHT recovery data alone is insufficient for stable fine-tuning.}
    In both first-flag and all-flag settings, new-only fine-tuning causes rapid forgetting. Mixing recovery data with prior demonstrations prevents collapse and preserves retained-task performance.
    }
    \label{fig:rq3_new_only_forgetting_strong_only}
\end{figure}

These results reveal the key tension of active VLA adaptation. Uncertainty-guided data is useful because it concentrates supervision on difficult states, but this same concentration makes the dataset distributionally narrow. Active learning for VLAs therefore cannot be treated only as a data-selection problem. It must also solve the continual-learning problem of integrating targeted new data without erasing previously learned behaviors.

\subsection{Low Learning Rates and EWC Expose a Stability-Plasticity Tradeoff}
\label{sec:results_ewc}

To address catastrophic forgetting, we evaluate whether smaller updates or parameter regularization can stabilize new-only adaptation. We compare standard new-only fine-tuning, low constant learning-rate fine-tuning, and elastic weight consolidation (EWC). EWC penalizes movement away from the original model parameters according to a Fisher information estimate, with larger coefficients placing stronger constraints on parameters deemed important for prior behavior.

Figure~\ref{fig:rq4_ewc_low_lr_tradeoff} compares representative EWC coefficients against low learning-rate fine-tuning and replay-based all-mix training. Low-learning-rate new-only training reaches 62.8\% overall success at its best checkpoint and preserves retained-task performance at 91.2\%, but collected-task success remains only 34.4\%. Similarly, EWC with $\lambda=10^{12}$ reaches 61.4\% overall success, with 32.0\% collected-task success and 90.8\% retained-task success. These methods preserve prior behavior but do not match replay-based mixing, which reaches 69.8\% overall success and 48.8\% collected-task success.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq4_ewc_low_lr_tradeoff.png}
    \caption{
    \textbf{Low learning rates and EWC reduce forgetting but limit adaptation.}
    Low learning-rate fine-tuning and EWC preserve retained-task performance better than standard new-only training, but they produce smaller gains on collected tasks than replay-based all-mix training.
    }
    \label{fig:rq4_ewc_low_lr_tradeoff}
\end{figure}

Figure~\ref{fig:rq4_ewc_low_lr_full_sweep} shows the full low-learning-rate EWC coefficient sweep. Across coefficients, EWC can maintain retained-task success near the original baseline for long training horizons, especially at high regularization strengths. However, collected-task performance remains limited, and overall success does not match replay-based all-mix training. This indicates that EWC can solve part of the problem---retention---but not the full active adaptation problem.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq4_ewc_low_lr_full_sweep.png}
    \caption{
    \textbf{Full EWC coefficient sweep with low learning rate.}
    Stronger Fisher regularization stabilizes retained-task performance, but the model does not gain enough plasticity to fully exploit uncertainty-guided recovery data.
    }
    \label{fig:rq4_ewc_low_lr_full_sweep}
\end{figure}

We also test filtered Fisher estimates, where the Fisher information is computed using a subset of prior data. Figure~\ref{fig:rq4_filtered_fisher_sweep} shows that filtered EWC produces similar qualitative behavior: regularization can stabilize parts of the model's prior behavior, but does not consistently recover the adaptation benefits of replay-based mixing. This suggests that the limitation is not only the choice of Fisher reference data, but also the broader difficulty of using parameter regularization alone to balance stability and plasticity in large autoregressive robot policies.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq4_filtered_fisher_sweep.png}
    \caption{
    \textbf{Filtered Fisher EWC sweep.}
    Computing Fisher information on filtered prior data changes the stability-plasticity behavior but does not remove the core tradeoff. Regularization preserves prior behavior more effectively than new-only training but does not match replay-based adaptation.
    }
    \label{fig:rq4_filtered_fisher_sweep}
\end{figure}

Overall, low learning rates and EWC expose a clear stability-plasticity tradeoff. Weak constraints allow adaptation but can forget prior behaviors, while strong constraints preserve prior behaviors but prevent the model from learning enough from recovery demonstrations. In our experiments, replay-based mixing provides the most reliable balance.

\subsection{Replay Scope Controls Adaptation and Retention}
\label{sec:results_replay_scope}

Since replay-based mixing is the most effective strategy, we next ask how much prior data must be replayed. Mixing with the full prior dataset is effective, but may be expensive as deployment histories grow. We therefore compare full prior-data replay, replay restricted to LIBERO-10 demonstrations, and replay restricted only to the LIBERO-10 tasks for which recovery data was collected.

Figure~\ref{fig:rq5_replay_scope_curves} shows training curves for these replay scopes. Full prior-data replay and LIBERO-10 replay both maintain strong retained-task performance while improving collected tasks. LIBERO-10 replay reaches 68.6\% overall success at its best checkpoint, close to the 69.8\% achieved by full prior-data replay. This suggests that replay may not require the entire prior dataset if the replay subset covers the behaviors needed for evaluation.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq5_replay_scope_curves.png}
    \caption{
    \textbf{Replay scope affects adaptation and retention over training.}
    Full prior-data replay and LIBERO-10 replay provide stable adaptation, while collected-task-only replay becomes less stable and degrades retained-task performance over training.
    }
    \label{fig:rq5_replay_scope_curves}
\end{figure}

Figure~\ref{fig:rq5_replay_scope_best_bars} summarizes the best checkpoint for each replay scope. LIBERO-10 replay reaches 68.6\% overall success, statistically indistinguishable from the 69.8\% achieved by full prior-data replay ($p=0.681$). This suggests that replay may not require the entire prior dataset when the replay subset covers the behaviors needed for evaluation. In contrast, collected-task-only replay reaches 63.2\% overall success and significantly reduces retained-task performance relative to LIBERO-10 replay, dropping from 90.0\% to 83.6\% retained-task success ($p=0.0345$). This indicates that replay data must include behaviors that should be preserved, not only the tasks for which new recovery demonstrations were collected.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq5_replay_scope_best_bars.png}
    \caption{
    \textbf{Best-checkpoint comparison of replay scope.}
    LIBERO-10 replay approaches the performance of full prior-data replay. Collected-task-only replay improves collected tasks but loses retained-task performance, showing that replay coverage matters for preserving prior capabilities.
    }
    \label{fig:rq5_replay_scope_best_bars}
\end{figure}

Finally, we evaluate whether EWC can stabilize the collected-task-only replay setting. Figure~\ref{fig:rq5_collected_replay_ewc} compares collected-task replay with several EWC and filtered-EWC variants. In this setting, EWC does not consistently solve the retention problem. Some variants briefly preserve performance early in training, but many runs later degrade substantially. This suggests that when replay coverage is too narrow, parameter regularization alone is not enough to compensate for missing retained-task data.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/rq5_collected_replay_ewc.png}
    \caption{
    \textbf{EWC does not reliably rescue collected-task-only replay.}
    We evaluate EWC and filtered-EWC variants when replay is restricted to the tasks for which recovery data was collected. Regularization does not consistently prevent degradation, indicating that replay coverage is critical.
    }
    \label{fig:rq5_collected_replay_ewc}
\end{figure}

These results clarify the role of replay in active continual VLA learning. Replay does not necessarily need to include the full original dataset, but it must cover the behaviors that should be retained. A replay set restricted only to newly targeted tasks can bias adaptation toward those tasks and allow performance on non-collected tasks to degrade.

\subsection{Summary of Findings}
\label{sec:results_summary}

Across these experiments, five findings emerge. First, uncertainty-guided recovery demonstrations are more informative than matched passive start-state recollection, showing that policy-induced uncertain states are useful targets for active data collection. Second, collecting from the first flagged state is more demonstration-efficient than collecting from all flagged states: dense all-flag collection does not provide a statistically significant overall advantage despite requiring more recovery demonstrations. Third, recovery data alone is not sufficient for fine-tuning; new-only training causes catastrophic forgetting, especially on retained tasks. Fourth, low learning rates and EWC reduce forgetting but expose a stability-plasticity tradeoff, preserving old behavior at the cost of reduced adaptation. Fifth, replay-based data mixing provides the strongest overall solution, but replay coverage matters: LIBERO-10 replay approaches full prior-data replay, while collected-task-only replay fails to preserve retained-task performance.

Together, these results support the central claim that active learning for VLAs must be formulated as active continual learning. INSIGHT-style help predictors can identify informative states for uncertainty-guided recovery collection, but the resulting data is narrow and distribution-shifted. Effective adaptation therefore requires both targeted data collection and mechanisms for preserving previously learned behaviors. In our experiments, replay-based mixing provides the most reliable balance between adapting to uncertainty-guided demonstrations and retaining prior task competence.
